Large Language Models on Graphs: A Comprehensive Survey

Large language models (LLMs), such as GPT4 and LLaMA, are creating significant advancements in natural language processing, due to their strong text encoding/decoding ability and newly found emergent capability (e.g., reasoning). While LLMs are mainly designed to process pure texts, there are many real-world scenarios where text data is associated with rich structure information in the form of graphs (e.g., academic networks, and e-commerce networks) or scenarios where graph data is paired with rich textual information (e.g., molecules with descriptions). Besides, although LLMs have shown their pure text-based reasoning ability, it is underexplored whether such ability can be generalized to graphs (i.e., graph-based reasoning). In this paper, we provide a systematic review of scenarios and techniques related to large language models on graphs. We first summarize potential scenarios of adopting LLMs on graphs into three categories, namely pure graphs, text-attributed graphs, and text-paired graphs. We then discuss detailed techniques for utilizing LLMs on graphs, including LLM as Predictor, LLM as Encoder, and LLM as Aligner, and compare the advantages and disadvantages of different schools of models. Furthermore, we discuss the real-world applications of such methods and summarize open-source codes and benchmark datasets. Finally, we conclude with potential future research directions in this fast-growing field. The related source can be found at https://github.com/PeterGriffinJin/Awesome-Language-Model-on-Graphs.

==> figure/hierarchy-v2.tex <==
\definecolor{connect-color}{RGB}{0,0,0}
\definecolor{middle-color}{RGB}{255,255,255}
% \definecolor{leaf-color}{RGB}{166,208,153}
\definecolor{leaf-color}{RGB}{173,216,230}
% \definecolor{line-color}{RGB}{166,208,153}
\definecolor{line-color}{RGB}{25,25,112}

\tikzstyle{leaf}=[draw=line-color,
    rounded corners,minimum height=1em,
    fill=leaf-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\tikzstyle{middle}=[draw=line-color,
    rounded corners,minimum height=1em,
    fill=middle-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\begin{figure*}[ht]
\centering
\begin{forest}
  for tree={
    forked edges,
    grow=east,
    reversed=true,
    anchor=base west,
    parent anchor=east,
    child anchor=west,
    base=middle,
    font=\scriptsize,
    rectangle,
    line width=0.9pt,
    draw=connect-color,
    rounded corners,align=left,
    minimum width=2em,
    s sep=5pt,
    inner xsep=3pt,
    inner ysep=1pt,
  },
  where level=1{text width=4.5em}{},
  where level=2{text width=6em,font=\scriptsize}{},
  where level=3{font=\scriptsize}{},
  where level=4{font=\scriptsize}{},
  where level=5{font=\scriptsize}{},
  [Categorization of LLM on Graph, middle,rotate=90,anchor=north,edge=connect-color
    [Pure Graphs, middle, edge=connect-color, text width=5em
        [LLM as Predictor, middle, edge=connect-color, text width=8.2em
            [Direct Answering, middle, text width=10.6em, edge=connect-color
                [Zero-Shot\cite{wang2023can, liu2023evaluating, guo2023gpt4graph, zhang2023llm4dyg, fatemi2023talk}{,} \\
                Few-Shot\cite{wang2023can, liu2023evaluating, zhang2023llm4dyg, fatemi2023talk}{,}
                GraphLLM\cite{chai2023graphllm}{,} \\
                Role Prompting\cite{guo2023gpt4graph}{,} Format Explanation\cite{guo2023gpt4graph}{,}, leaf, text width=17.7em, edge=connect-color]
            ]
            [Heuristic Reasoning, middle, text width=10.6em, edge=connect-color
                [CoT\cite{wang2023can, liu2023evaluating, guo2023gpt4graph, zhang2023llm4dyg, fatemi2023talk, sun2023think}{,}\\
                Self-Consistency\cite{wang2023can}{,} BaG\cite{wang2023can, fatemi2023talk}{,} \\
                RoG\cite{luo2023reasoning}{,} StructGPT\cite{jiang2023structgpt}{,} ToG\cite{sun2023think}
                , leaf, text width=17.7em, edge=connect-color]
            ]
            [Algorithmic Reasoning, middle, text width=10.6em, edge=connect-color
                [Algorithmic Prompting\cite{wang2023can}{,} 
                Graph-ToolFormer\cite{zhang2023graph}, leaf, text width=17.7em, edge=connect-color]
            ]
        ]
    ]
    [Text-Rich \\ Graphs, middle, edge=connect-color, text width=5em
        [LLM as Predictor, middle, edge=connect-color,text width=8.2em
            [Graph as \\ Sequence, middle, text width=4.2em, edge=connect-color
                [Rule-based, middle, text width=4.5em, edge=connect-color
                    [InstructGLM \cite{ye2023natural}{,}  GraphText \cite{zhao2023graphtext}{,} \cite{huang2023can}{,}, leaf, text width=17.7em, edge=connect-color]
                ]
                [GNN-based, middle, text width=4.5em, edge=connect-color
                    [GNP \cite{tian2023graph}{,} GraphGPT \cite{tang2023graphgpt}{,} DGTL \cite{qin2023disentangled}{,} METERN \cite{jin2023learning} , leaf, text width=17.7em, edge=connect-color]
                ]
            ]
            [Graph-Empowered LLM, middle, text width=10.6em, edge=connect-color
                [GreaseLM \cite{zhang2022greaselm}{,} DRAGON \cite{yasunaga2022deep}{,} GraphFormers \cite{yang2021graphformers}{,}\\ Patton \cite{jin2023patton}{,} Heterformer \cite{jin2023heterformer}{,} Edgeformers \cite{jin2023edgeformers}{,}, leaf, text width=17.7em, edge=connect-color]
            ]
            [Graph-Aware LLM Finetuning, middle, text width=10.6em, edge=connect-color
                [SPECTER \cite{cohan2020specter}{,} SciNCL \cite{ostendorff2022neighborhood}{,} Touchup-G \cite{zhu2023touchup}{,} \\ TwHIN-BERT \cite{zhang2023twhin}{,} MICoL \cite{zhang2022metadata}{,} E2EG \cite{dinh2022e2eg} , leaf, text width=17.7em, edge=connect-color]
            ]
        ]
        [LLM as Encoder, middle, edge=connect-color, text width=8.2em
            [Optimization, middle, text width=4.5em, edge=connect-color
                [One-step, middle, text width=4.2em, edge=connect-color
                [TextGNN \cite{zhu2021textgnn}{,} AdsGNN \cite{li2021adsgnn}{,} GNN-LM \cite{meng2021gnn}, leaf, text width=17.7em, edge=connect-color]
                ]
                [Two-step, middle, text width=4.2em, edge=connect-color
                    [GIANT \cite{chien2021node}{,} LM-GNN \cite{ioannidis2022efficient}{,} SimTeG \cite{duan2023simteg}{,} GaLM \cite{xie2023graph}, leaf, text width=17.7em, edge=connect-color]
                ]
            ]
            % [Joint Training, middle, text width=10.8em, edge=connect-color
            %     [TextGNN \cite{zhu2021textgnn}{,} AdsGNN \cite{li2021adsgnn}{,} GNN-LM \cite{meng2021gnn}, leaf, text width=17.5em, edge=connect-color]
            % ]
            % [Two-step Training, middle, text width=10.8em, edge=connect-color
            %     [GIANT \cite{chien2021node}{,} LM-GNN \cite{ioannidis2022efficient}{,} SimTeG \cite{duan2023simteg}{,} GaLM \cite{xie2023graph}, leaf, text width=17.5em, edge=connect-color]
            % ]
            [Data Augmentation, middle, text width=10.6em, edge=connect-color
                [LLM-GNN \cite{chen2023label}{,} TAPE \cite{he2023explanations}{,} ENG \cite{yu2023empower}, leaf, text width=17.7em, edge=connect-color]
            ]
            [Knowledge Distillation, middle, text width=10.6em, edge=connect-color
                [AdsGNN \cite{li2021adsgnn}{,} GraD \cite{mavromatis2023train}, leaf, text width=17.7em, edge=connect-color]
            ]
        ]
        [LLM as Aligner, middle, edge=connect-color, text width=8.2em
            [Prediction Alignment, middle, text width=10.6em, edge=connect-color
                [LTRN \cite{zhang2021minimally}{,} GLEM \cite{zhao2022learning}, leaf, text width=17.7em, edge=connect-color]
            ]
            [Latent Space Alignment, middle, text width=10.6em, edge=connect-color
                [ConGrat \cite{brannon2023congrat}{,}  GRENADE \cite{li2023grenade}{,} G2P2 \cite{wen2023augmenting}{,} THLM \cite{zou2023pretraining} ,leaf, text width= 17.7em, edge=connect-color]
            ]
        ]
    ]
    [Text-Paired \\ Graphs, middle, edge=connect-color, text width=5em
        [LLM as Predictor, middle, edge=connect-color, text width=8.2em
            [Graph as Sequence, middle, text width=10.6em, edge=connect-color
                [CatBERTa~\cite{catberta} {,} LLaMA-Mol~\cite{llamamol} {,} LLM4Mol~\cite{llm4mol} {,} \\ RT~\cite{regt} {,} MolReGPT~\cite{molregpt} {,} ChatMol~\cite{chatmol} {,} \\  MolXPT~\cite{molxpt} {,} LLM-ICL~\cite{llmicl} {,} Text+Chem T5~\cite{tct} {,} \\ MolT5~\cite{edwards2022translation} {,} KV-PLM~\cite{kvplm} {,} Chemformer~\cite{chemformer} {,} \\ MFBERT~\cite{mfbert} {,} Galatica~\cite{galatica} {,} SMILES-BERT~\cite{smilesbert} , leaf, text width=17.7em, edge=connect-color]
            ]
            [Graph-Empowered LLM, middle, text width=10.6em, edge=connect-color
                [ReLM~\cite{relm} {,} Prot2Text~\cite{prot2text} {,} GIMLET~\cite{zhao2023gimlet} {,} \\ Text2Mol~\cite{edwards2021text2mol} ,leaf, text width= 17.7em, edge=connect-color]
            ]
        ]
        [LLM as Aligner, middle, edge=connect-color, text width=8.2em
            [Latent Space Alignment, middle, text width=10.6em, edge=connect-color
                [MolCA~\cite{molca} {,} GIT-Mol~\cite{gitmol} {,} MolFM~\cite{molfm} {,} \\ CLAMP~\cite{clamp} {,} MoMu-v2~\cite{momuv2} {,} MoleculeSTM~\cite{moleculestm} {,} \\ MoMu~\cite{momu} ,leaf, text width= 17.7em, edge=connect-color]
            ]
        ]
    ]
  ]  
\end{forest}
\caption{A taxonomy of LLM on graph scenarios and techniques with representative examples.}
\label{fig:taxonomy-techniques}
\end{figure*}

% Prof. Jiang: make the final layer in the taxonomy more clear
% Utilizing LM to enhance features in GM
% graph is too complex, embedding is complex
% a diagram for the second layer
% third-level diagram (augmentation, distillation, joint/two-step training)


% Graph as Implicit Inputs
% Graph as Feature Sources
% Graph as Alignment Signals

% LM to output
% LM as initial encoder
% LM to be aligned


==> figure/hierarchy.tex <==
\tikzstyle{leaf}=[draw=hiddendraw,
    rounded corners,minimum height=1em,
    fill=mygreen!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\tikzstyle{middle}=[draw=hiddendraw,
    rounded corners,minimum height=1em,
    fill=output-white!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\begin{figure*}[ht]
\centering
\begin{forest}
  for tree={
  forked edges,
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=middle,
  font=\scriptsize,
  rectangle,
  line width=0.7pt,
  draw=output-black,
  rounded corners,align=left,
  minimum width=2em,
  % minimum height=1em,
    s sep=5pt,
    inner xsep=3pt,
    inner ysep=1pt,
  },
  where level=1{text width=4.5em}{},
  where level=2{text width=6em,font=\scriptsize}{},
  where level=3{font=\scriptsize}{},
  where level=4{font=\scriptsize}{},
  where level=5{font=\scriptsize}{},
  [LM on Graph Techniques, middle,rotate=90,anchor=north,edge=output-black
    [LM-Centric: Encoding Graph \\ into LM, middle, edge=output-black,text width=11.2em
        [Graph-aware LM Finetuning, middle, text width=10.8em, edge=output-black
            [SPECTER \cite{cohan2020specter}{,} SciNCL \cite{ostendorff2022neighborhood}{,} Touchup-G \cite{zhu2023touchup}{,} \\ TwHIN-BERT \cite{zhang2023twhin}{,} MICoL \cite{zhang2022metadata}{,} E2EG \cite{dinh2022e2eg} , leaf, text width=17.5em, edge=output-black]
        ]
        [Graph2Seq, middle, text width=4.2em, edge=output-black
            [Rule-based, middle, text width=4.7em, edge=output-black
                [InstructGLM \cite{ye2023natural}{,}  GraphText \cite{zhao2023graphtext}{,} \cite{huang2023can}{,} \\  xxxx, leaf, text width=17.5em, edge=output-black]
            ]
            [GM-based, middle, text width=4.7em, edge=output-black
                [GNP \cite{tian2023graph}{,} GraphGPT \cite{tang2023graphgpt}{,} DGTL \cite{qin2023disentangled}{,} METERN \cite{jin2023learning} \\
                xxx , leaf, text width=17.5em, edge=output-black]
            ]
        ]
        [Graph-Empowered Transformers, middle, text width=10.8em, edge=output-black
            [GreaseLM \cite{zhang2022greaselm}{,} DRAGON \cite{yasunaga2022deep}{,} GraphFormers \cite{yang2021graphformers}{,}\\ Patton \cite{jin2023patton}{,} Heterformer \cite{jin2023heterformer}{,} Edgeformers \cite{jin2023edgeformers}{,}\\ xxx, leaf, text width=17.5em, edge=output-black]
        ]
    ]
    [GM-Centric: Utilizing LM \\ as Feature Extractor, middle, edge=output-black, text width=11.2em
        [Joint Training, middle, text width=10.8em, edge=output-black
            [TextGNN \cite{zhu2021textgnn}{,} AdsGNN \cite{li2021adsgnn}{,} GNN-LM \cite{meng2021gnn}, leaf, text width=17.5em, edge=output-black]
        ]
        [Two-step Training, middle, text width=10.8em, edge=output-black
            [GIANT \cite{chien2021node}{,} LM-GNN \cite{ioannidis2022efficient}{,} SimTeG \cite{duan2023simteg}{,} GaLM \cite{xie2023graph}, leaf, text width=17.5em, edge=output-black]
        ]
        [Augmentation, middle, text width=10.8em, edge=output-black
            [LLM-GNN \cite{chen2023label}{,} TAPE \cite{he2023explanations}{,} ENG \cite{yu2023empower}, leaf, text width=17.5em, edge=output-black]
        ]
        [Distillation, middle, text width=10.8em, edge=output-black
            [AdsGNN \cite{li2021adsgnn}{,} GraD \cite{mavromatis2023train}, leaf, text width=17.5em, edge=output-black]
        ]
    ]
    [LM-GM Cycled/Aligned: \\ Achieving Unified Representation, middle, edge=output-black, text width=11.2em
        [Iterative, middle, text width=10.8em, edge=output-black
            [LTRN \cite{zhang2021minimally}{,} GLEM \cite{zhao2022learning}{,} xxx, leaf, text width=17.5em, edge=output-black]
        ]
        [Contrastive, middle, text width=10.8em, edge=output-black
            [ConGrat \cite{brannon2023congrat}{,}  GRENADE \cite{li2023grenade}{,} G2P2 \cite{wen2023augmenting}{,} THLM \cite{zou2023pretraining}{,} \\ xxx ,leaf, text width= 17.5em, edge=output-black]
        ]
    ]
  ]  
\end{forest}
\caption{A taxonomy of LM on graph techniques with representative examples. \bowen{add more examples}}
\label{fig:taxonomy-techniques}
\end{figure*}


==> tables/5.node-text-model.tex <==

\begin{table*}[htb]
\caption{Summary of language models on graphs with node/edge-level textual information. Role of LM: ``TE'', ``SE'', ``ANN'' and ``AUG'' denote text encoder, structure encoder, annotator (labeling the node/edges), and augmentator (conduct data augmentation). Task: ``NC'', ``UAP'', ``LP'', ``Rec'', ``QA'', ``NLU'', ``EC'', ``LM'', ``RG'' denote node classification, user activity prediction, link prediction, recommendation, question answering natural language understanding, edge classification, language modeling, and regression task.}\label{tab:category}
\centering
\begin{adjustbox}{width=0.90\textwidth}
\begin{tabular}{llllllll}
\toprule
Approach & Time & Category & Role of LM & LM Size & Focus & Task & Data \\ \midrule
GNN-LM \cite{meng2021gnn} & 2021.10 & GNN-centric & TE & 237M & Task & LM & WikiText-103, One Billion Word, Enwik8 \\ \midrule
GIANT \cite{chien2021node} & 2021.11 & GNN-centric & TE & 110M & Task & NC & ogb-arxiv/products/papers110M \\ \midrule
TextGNN \cite{zhu2021textgnn} & 2022.1 & GNN-centric & TE & 110M & Task & Search & internal industry dataset \\ \midrule
AdsGNN \cite{li2021adsgnn} & 2022.4 & GNN-centric & TE & 110M & Task & Search & internal industry dataset \\ \midrule
LM-GNN \cite{ioannidis2022efficient} & 2022.6 & GNN-centric & TE & 110M & Efficiency & NC, LP, EC & ogb-arxiv, ogb-product \\ \midrule
GraD \cite{mavromatis2023train} & 2023.4 & GNN-centric & TE & 110M/66M & Efficiency & LP, NC & ogb-arxiv, ogb-products, ogb-papers110M \\ \midrule
TAPE \cite{he2023explanations} & 2023.5 & GNN-centric & TE, AUG & 129M/GPT-3.5 & Task & NC & cora, PubMed, ogb-arxiv/product, tape-arxiv23 \\ \midrule
SimTeG \cite{duan2023simteg} & 2023.8 & GNN-centric & TE & 80M/355M & Task & NC, LP & ogb-arxiv/products/citation2 \\ \midrule
LLM-GNN \cite{chen2023label} & 2023.10 & GNN-centric & ANN & GPT-3.5 & Task & NC & Cora, Citeseer, Pubmed, ogb-arxiv/products \\ \midrule
ENG \cite{yu2023empower} & 2023.10 & GNN-centric & TE, AUG & 80M/GPT-3.5 & Task & NC & cora, PubMed, ogb-arxiv \\ \midrule
SPECTER \cite{cohan2020specter} & 2020.4 & LM-centric & TE & 110M & Representation & NC, UAP, LP, Rec & SciDocs \footnote{https://github.com/allenai/scidocs} \\ \midrule
GraphFormers \cite{yang2021graphformers} & 2021.5 & LM-centric & TE, SE & 110M & Representation & LP & DBLP \footnote{6https://originalstatic.aminer.cn/misc/dblp.v12.7z}, Wikidata5M \footnote{https://deepgraphlearning.github.io/project/wikidata5m}   \\ \midrule
GreaseLM \cite{zhang2022greaselm} & 2022.1 & LM-centric & TE, SE & 355M & Task & QA & CommonsenseQA, OpenbookQA, MedQA-USMLE \\ \midrule
SciNCL \cite{ostendorff2022neighborhood} & 2022.2 & LM-centric & TE & 110M & Representation & NC, UAP, LP, Rec & SciDocs \footnote{https://github.com/allenai/scidocs} \\ \midrule
MICoL \cite{zhang2022metadata} & 2022.2 & LM-centric & TE & 110M & Supervision & NC & MAG-CS, PubMed \\ \midrule
LinkBERT \cite{yasunaga2022linkbert} & 2022.3 & LM-centric & TE & 110M & Pretraining & QA, NLU & MRQ \footnote{https://huggingface.co/datasets/mrqa}, GLUE \footnote{https://gluebenchmark.com/} \\ \midrule
Heterformer \cite{jin2023heterformer} & 2022.5 & LM-centric & TE, SE & 110M & Representation & NC, LP & DBLP, Twitter, Goodreads   \\ \midrule
E2EG \cite{dinh2022e2eg} & 2022.8 & LM-centric & TE & 66M & Task & NC & ogb-arxiv/products \\ \midrule
TwHIN-BERT \cite{zhang2023twhin} & 2022.9 & LM-centric & TE & 110M/355M & Pretraining & NC, LP & Twitter \\ \midrule
Edgeformers \cite{jin2023edgeformers} & 2023.1 & LM-centric & TE, SE & 110M & Representation & NC, LP, EC & Amazon, Goodreads, Stackoverflow   \\ \midrule
Patton \cite{jin2023patton} & 2023.5 & LM-centric & TE, RE & 110M & Pretraining & NC, LP, Search & MAG, Amazon   \\ \midrule
InstructGLM \cite{ye2023natural} & 2023.8 & LM-centric & TE, SE & 250M/7B & Generalization & NC, LP & Cora, PubMed, ogb-arxiv \\ \midrule
GNP \cite{tian2023graph} & 2023.9 & LM-centric & TE, SE & 3B/11B & Task & QA & OBQA, ARC, PIQA, Riddle, PubMedQA, BioASQ \\ \midrule
Touchup-G \cite{zhu2023touchup} & 2023.9 & LM-centric & TE & 110M & Representation & NC, LP & Books, OGB-Products, Amazon-CP, OGB-Arxiv \\ \midrule
DGTL \cite{qin2023disentangled} & 2023.10 & LM-centric & TE, SE & 13B & Task & NC & Cora, PubMed, Books   \\ \midrule
GraphText \cite{zhao2023graphtext} & 2023.10 & LM-centric & TE, SE & GPT-3.5/4 & Task & NC & cora \footnote{https://relational.fit.cvut.cz/dataset/CORA}, citeseer \footnote{https://linqs.soe.ucsc.edu/data}, texas \footnote{https://docs.dgl.ai/en/0.8.x/api/python/dgl.data.html\#node-prediction-datasets}, Wisconsin \footnote{https://docs.dgl.ai/en/0.8.x/api/python/dgl.data.html\#node-prediction-datasets}, cornell \footnote{https://docs.dgl.ai/en/0.8.x/api/python/dgl.data.html\#node-prediction-datasets} \\ \midrule
GraphGPT \cite{tang2023graphgpt} & 2023.10 & LM-centric & TE, SE & 7B & Generalization & NC & ogb-arxiv, PubMed, cora \\ \midrule
METERN \cite{jin2023learning} & 2023.10 & LM-centric & TE, RE & 110M & Representation & NC, LP, Rec, RG & MAG, Amazon   \\ \midrule
LTRN \cite{zhang2021minimally} & 2021.2 & parallel & TE & 110M & Supervision & NC & Amazon, Books \\ \midrule
GLEM \cite{zhao2022learning} & 2023.1 & parallel & TE & 110M & Task & NC & ogb-arxiv/product/paper \\ \midrule
G2P2 \cite{wen2023augmenting} & 2023.5 & parallel & TE & 110M & Supervision & NC & Cora, Amazon \\ \midrule
ConGraT \cite{brannon2023congrat} & 2023.5 & parallel & TE & 110M/82M & Representation & LP, LM, NC & Pubmed, T-REx, Twitter \footnote{https://github.com/wwbrannon/congrat/tree/master/data} \\ \midrule
GRENADE \cite{li2023grenade} & 2023.10 & parallel & TE & 110M & Representation & NC, LP & OGB-arxiv/products/citations2 \\ \midrule
THLM \cite{zou2023pretraining} & 2023.10 & parallel & TE & 110B & Pretraining & NC, LP & OGB-Venue, Goodreads, Patents   \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> tables/6.graph-text-data-complete.tex <==
\begin{table*}
    \centering
    \caption{\footnotesize Data collection in Section \ref{sec:graph-text} for text-captioned graphs. The availability of text refers to the text descriptions of graphs, not the format of the linearized graphs like the SMILES-represented molecules. ``PT'', ``FT'', ``Cap.'', ``GC'', ``Retr.', ``Gen.'', and ``GR'' refer to pretraining, finetuning, caption, graph classification, retrieval, graph generation, graph regression, respectively. The superscript for the size denotes \# graph-text pairs$^1$, \# graphs$^2$, \# assays$^3$.}
    \label{tab:graph-text-data}
    \begin{adjustbox}{width=0.75\textwidth}
    \begin{tabular}{lllllll}
    \toprule
    & Data & Date & Task & Size & Tested Model & Source \& Notes \\
    \midrule
    \multirow{24}{*}{\rotatebox{90}{\normalsize Both Graph and Text Are Available}}
    & ChEMBL-2023~\cite{chembl2023} & 2023 & Various & 2.4M$^2$,20.3M$^3$ & Various & Drug-like \\
    \cmidrule(l){2-7}
    & PubChem~\cite{pubchem2019} & 2019 & Various & 96M$^2$,237M$^3$ & Various & Biomedical \\ 
    % \cmidrule(l){2-7}
    % & ChEMBL-2012~\cite{chembl2012} & 2012 & Various & 1M$^2$,5.4M$^3$ & Various & Drug-like \\
    \cmidrule(l){2-7}
    & \multirow{2}{*}{PC324K~\cite{molca}} & \multirow{2}{*}{2023} & PT & \multirow{2}{*}{324K$^1$} & \multirow{2}{*}{MolCA~\cite{molca}} & \multirow{2}{*}{PubChem~\cite{pubchem2019}} \\
    & & & Cap. & & & \\
    \cmidrule(l){2-7}
    & \multirow{3}{*}{MolXPT-PT~\cite{molxpt}} & \multirow{3}{*}{2023} & \multirow{3}{*}{PT} & \multirow{3}{*}{30M$^2$} & \multirow{3}{*}{MolXPT~\cite{molxpt}} & PubChem~\cite{pubchem2019}, \\
    & & & & & & PubMed, \\
    & & & & & & ChEBI~\cite{chebi} \\
    \cmidrule(l){2-7}
    & ChE-bio~\cite{zhao2023gimlet} & 2023 & PT & 365K$^2$ & GIMLET~\cite{zhao2023gimlet} & ChEMBL~\cite{chembl2012} \\
    \cmidrule(l){2-7}
    & ChE-phy~\cite{zhao2023gimlet} & 2023 & PT & 365K$^2$  & GIMLET~\cite{zhao2023gimlet} & ChEMBL~\cite{chembl2012} \\
    \cmidrule(l){2-7}
    & ChE ZS~\cite{zhao2023gimlet} & 2023 & GC & 91K$^2$ & GIMLET~\cite{zhao2023gimlet} & ChEMBL~\cite{chembl2012} \\
    \cmidrule(l){2-7}
    & \multirow{2}{*}{PC223M~\cite{clamp}} & \multirow{2}{*}{2023} & \multirow{1}{*}{PT} & \multirow{1}{*}{223M$^1$,2M$^2$,} & \multirow{2}{*}{CLAMP~\cite{clamp}} & \multirow{2}{*}{PubChem~\cite{pubchem2019}} \\
    & & & Retr. & 20K$^3$ & & \\
    \cmidrule(l){2-7}
    & PCSTM~\cite{moleculestm} & 2022 & PT & 281K$^1$ & MoleculeSTM~\cite{moleculestm} & PubChem~\cite{pubchem2019} \\
    \cmidrule(l){2-7}
    & \multirow{3}{*}{PCdes~\cite{pubchem2019}}& \multirow{3}{*}{2022} & FT, & \multirow{3}{*}{15K$^1$}
    & KV-PLM~\cite{kvplm}, MoMu~\cite{momu}, MolFM~\cite{molfm},
    & \multirow{3}{*}{PubChem~\cite{pubchem2019}} \\
    & & & Cap. & & \multirow{2}{*}{ChatMol~\cite{chatmol}, MolCA~\cite{molca}} & \\
    & & & Retr. & & & \\
    \cmidrule(l){2-7}
    % & BC5CDR & TODO & NER & TODO & KV-PLM~\cite{kvplm} & Chemical-disease  \\
    % \cmidrule(l){2-7}
    % & ChemProt & TODO & RE & TODO & KV-PLM~\cite{kvplm} & TODO \\
    % \cmidrule(l){2-7}
    & \multirow{4}{*}{ChEBI-20~\cite{edwards2021text2mol}} & \multirow{4}{*}{2021} & FT. &  \multirow{4}{*}{33K$^1$} 
    & Text2Mol~\cite{edwards2021text2mol}, MoMu~\cite{momu}, Text+Chem T5~\cite{tct},
    & \multirow{2}{*}{PubChem~\cite{pubchem2019}} \\
    & & & Retr. & & LLM-ICL~\cite{llmicl}, MolXPT~\cite{molxpt}, MolFM~\cite{molfm}, & \multirow{2}{*}{ChEBI~\cite{chebi}} \\
    & & & Gen. & & ChatMol~\cite{chatmol}, MolReGPT~\cite{molregpt}, & \\
    & & & Cap. & & GIT-Mol~\cite{gitmol}, MolCA~\cite{molca} & \\
    \midrule
    % \parbox[t]{2mm}{\multirow{30}{*}{\rotatebox[origin=c]{90}{Graph only}}}
    \multirow{40}{*}{\rotatebox{90}{\normalsize Graph only}}
    & ZINC15~\cite{zinc15} & 2015 & PT & 120M$^2$ & Various & Drug-like \\
    \cmidrule(l){2-7}
    & GDB13~\cite{gdb13} & 2009 & PT & 977M$^2$ & MFBERT~\cite{mfbert} & Drug-like \\
    \cmidrule(l){2-7}
    & FS-Mol~\cite{fs-mol} & 2021 & GC & 27,065$^2$ & CLAMP~\cite{clamp} & ChEMBL~\cite{chembl2012} \\
    \cmidrule(l){2-7}
    & PCBA~\cite{moleculenet} & 2018 & GC & 439,863$^2$ & SMILES-BERT~\cite{smilesbert}, GIMLET~\cite{zhao2023gimlet} & PubChem-Bio~\cite{pubchem2019} \\
    \cmidrule(l){2-7}
    & MUV~\cite{moleculenet} & 2018 & GC & 93,127$^2$ & MoMu~\cite{momu}, GIMLET~\cite{zhao2023gimlet}, MolFM~\cite{molfm} & PubChem-Bio~\cite{pubchem2019}  \\
    \cmidrule(l){2-7}
    & \multirow{3}{*}{HIV~\cite{moleculenet}} & \multirow{3}{*}{2018} & \multirow{3}{*}{GC} & \multirow{3}{*}{41,913$^2$} 
    & KV-PLM~\cite{kvplm}, MoMu~\cite{momu}, LLM-ICL~\cite{llmicl}, & \multirow{1}{*}{Drug Therapeutics}  \\
    & & & & &  MolXPT~\cite{molxpt}, CLAMP~\cite{clamp} & Program AIDS Antiviral \\
    & & & & &  GIMLET~\cite{zhao2023gimlet}, MolFM~\cite{molfm} & Screen Data~\cite{hivsource} \\
    \cmidrule(l){2-7}
    & CYP450~\cite{cyp450} & 2018 & GC & 16,896$^2$ & GIMLET~\cite{zhao2023gimlet} & Pharmacokinetic  \\
    \cmidrule(l){2-7}
    & \multirow{4}{*}{BACE~\cite{moleculenet}} & \multirow{4}{*}{2018} & \multirow{4}{*}{GC} & \multirow{4}{*}{1,522$^2$} & Galatica~\cite{galatica}, MoMu~\cite{momu}, MoMu-v2~\cite{momuv2}, & \multirow{1}{*}{Binding for}  \\
    & & & & &  LLM-ICL~\cite{llmicl}, MolXPT~\cite{molxpt}, CLAMP~\cite{clamp}, & inhibitors of \\
    & & & & &  GIMLET~\cite{zhao2023gimlet}, MolFM~\cite{molfm}, & human $\beta$-secretase 1 \\
    & & & & &  GIT-Mol~\cite{gitmol}, MolCA~\cite{molca} & ~\cite{bacesource} \\
    \cmidrule(l){2-7}
    & \multirow{4}{*}{BBBP~\cite{moleculenet}} & \multirow{4}{*}{2018 } & \multirow{4}{*}{GC} & \multirow{4}{*}{2,053$^2$}
    & Galatica~\cite{galatica}, KV-PLM~\cite{kvplm}, MoMu~\cite{momu},
    & \multirow{1}{*}{Blood-brain barrier}  \\
    & & & & &  MoMu-v2~\cite{momuv2}, LLM-ICL~\cite{llmicl}, MolXPT~\cite{molxpt}, & penetration \\
    & & & & &  CLAMP~\cite{clamp}, GIMLET~\cite{zhao2023gimlet}, MolFM~\cite{molfm}, & permeability\\
    & & & & &  GIT-Mol~\cite{gitmol}, MolCA~\cite{molca}, & \cite{bbbpsource} \\
    \cmidrule(l){2-7}
    & \multirow{4}{*}{Tox21~\cite{moleculenet}} & \multirow{4}{*}{2018} & \multirow{4}{*}{GC} & \multirow{4}{*}{8,014$^2$} & Galatica~\cite{galatica}, KV-PLM~\cite{kvplm}, MoMu~\cite{momu}, & \multirow{1}{*}{Toxicology in the}  \\
    & & & & &   MoMu-v2~\cite{momuv2}, LLM-ICL~\cite{llmicl}, MolXPT~\cite{molxpt}, & 21st Century \\
    & & & & &  CLAMP~\cite{clamp}, GIMLET~\cite{zhao2023gimlet}, MolFM~\cite{molfm}, & initiative \\
    & & & & &  GIT-Mol~\cite{gitmol}, MolCA~\cite{molca} & ~\cite{tox21source} \\
    \cmidrule(l){2-7}
    & \multirow{3}{*}{Toxcast~\cite{moleculenet}} & \multirow{3}{*}{2018} & \multirow{3}{*}{GC} & \multirow{3}{*}{8,615$^2$} & MoMu~\cite{momu}, MoMu-v2~\cite{momuv2}, CLAMP~\cite{clamp},  & \multirow{1}{*}{Toxicology in the}  \\
    & & & & & GIMLET~\cite{zhao2023gimlet}, MolFM~\cite{molfm}, & 21st Century \\
    & & & & & GIT-Mol~\cite{gitmol}, MolCA~\cite{molca} & initiative~\cite{tox21source }\\
    \cmidrule(l){2-7}
    & \multirow{3}{*}{SIDER~\cite{moleculenet}} & \multirow{3}{*}{2018} & \multirow{3}{*}{GC} & \multirow{3}{*}{1,427$^2$} & Galatica~\cite{galatica}, KV-PLM~\cite{kvplm}, MoMu~\cite{momu}, & \multirow{1}{*}{DeepChem~\cite{deepchem} for }  \\
    & & & & & MoMu-v2~\cite{momuv2}, MolXPT~\cite{molxpt}, MolFM~\cite{molfm}, & side effect resource \\
    & & & & & LLM4Mol~\cite{llm4mol}, GIT-Mol~\cite{gitmol}, MolCA~\cite{molca} & of marketed drugs \\
    \cmidrule(l){2-7}
    & \multirow{4}{*}{ClinTox~\cite{moleculenet}} & \multirow{4}{*}{2018} & \multirow{4}{*}{GC} & \multirow{4}{*}{1,491$^2$} 
    & Galatica~\cite{galatica}, MoMu~\cite{momu}, MoMu-v2~\cite{momuv2}, & \multirow{1}{*}{Drugs approved by}  \\
    & & & & & LLM-ICL~\cite{llmicl}, MolXPT~\cite{molxpt}, CLAMP~\cite{clamp}, & FDA or failed \\
    & & & & & MolFM~\cite{molfm}, LLM4Mol~\cite{llm4mol}, GIT-Mol~\cite{gitmol}, & clinical trials \\
    & & & & & MolCA~\cite{molca} & \cite{clintox1,clintox2}  \\
    \cmidrule(l){2-7}
    & Lipophilicity~\cite{moleculenet} & 2018  & GR & 4,200$^2$  & Chemformer~\cite{chemformer}, GIMLET~\cite{zhao2023gimlet}, LLM4Mol~\cite{llm4mol} & ChEMBL~\cite{chembl2012} \\
    \cmidrule(l){2-7}
    & ESOL~\cite{moleculenet} & 2018 & GR & 1,128$^2$ & Chemformer~\cite{chemformer}, GIMLET~\cite{zhao2023gimlet}, LLM4Mol~\cite{llm4mol} & \cite{esolsource} \\
    \cmidrule(l){2-7}
    & FreeSolv~\cite{moleculenet} & 2018 & GR & 642$^2$ & Chemformer~\cite{chemformer}, GIMLET~\cite{zhao2023gimlet} & \cite{freesolvsource} \\
    % \midrule
    % & USPTO & X & Reac. & 479K & LLM-ICL~\cite{llmicl}, ReLM~\cite{relm} & \\
    % \cmidrule(l){2-7}
    % & Pistachio & X & Reac. & 2.3M & Text+Chem T5~\cite{tct} & X \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

==> tables/6.graph-text-model-v2.tex <==
\begin{table*}[htb]
    \centering
    \caption{Model collection in Section~\ref{sec:graph-text} for addressing textual information on graph levels. ``Lin.'' and ``Vec.'' represent Linearized Graph Encoding and Vectorized Graph Encoding. ``Classif.'', ``Regr.'', ``NER'', ``RE'', ``Retr.'', ``Gen.'', ``Cap.'' represent classification, regression, named entity recognition, relation extraction, (molecule) graph retrieval, (molecule) graph generation, (molecule) graph captioning.}
    \label{tab:graph-text-model-v2}
    \begin{adjustbox}{width=0.90\textwidth}
    \begin{tabular}{llllllll}
    \toprule
        Model & Time & Category & LM Encoder & Graph Encoder & Generation Decoder & LM Size & Task\\
        \midrule
        ReLM~\cite{relm} & 2023.10 & LM-Centric & N.A. & GNN & GPT-3.5 & N.A. & Classification \\
        \midrule
        CatBERTa~\cite{catberta} & 2023.10 & LM-Centric & N.A. & Linearized & RoBERTa~\cite{roberta} & N.A. & Regression \\
        \midrule
        LLaMA-Mol~\cite{llamamol} & 2023.07 & LM-Centric & N.A. & Linearized & LLaMA & 7B & Regr., Gene. \\
        \midrule
        LLM4Mol~\cite{llm4mol} & 2023.07 & LM-Centric & RoBERTa~\cite{roberta} & Linearized & GPT-3.5 & N.A. & Classif, Regr. \\
        \midrule
        RT~\cite{regt} & 2023.06 & LM-Centric & N.A. & Linearized & XLNet & 27M & Regr. Gen. \\
        \midrule
        MolReGPT~\cite{molregpt} & 2023.06 & LM-Centric & N.A. & Linearized & GPT-3.5 & N.A. & Gen., Cap.\\
        \midrule
        ChatMol~\cite{chatmol} & 2023.06 & LM-Centric & T5~\cite{T5} & Linearized & T5 & 80M-780M & Gen., Cap. \\
        \midrule
        \multirow{2}{*}{MolXPT~\cite{molxpt}} & \multirow{2}{*}{2023.05} & \multirow{2}{*}{LM-Centric} & \multirow{2}{*}{N.A.} & \multirow{2}{*}{Linearized} & \multirow{2}{*}{GPT-2} & \multirow{2}{*}{350M} & Classif, Gen., \\
        & & & & & & &  Caption \\
        \midrule
        \multirow{3}{*}{LLM-ICL~\cite{llmicl}} & \multirow{3}{*}{2023.05} & \multirow{3}{*}{LM-Centric} & \multirow{3}{*}{N.A.} & \multirow{3}{*}{Linearized} & GPT-3.5/4 & \multirow{3}{*}{$\geq$ 780M} & Classification \\
        & & & & & LLaMA2 & & Generation \\
        & & & & & Galactica & & Caption \\
        \midrule
        \multirow{2}{*}{Text+Chem T5~\cite{tct}} & \multirow{2}{*}{2023.05} & \multirow{2}{*}{LM-Centric} & \multirow{2}{*}{T5~\cite{T5}} & \multirow{2}{*}{Linearized} & \multirow{2}{*}{T5} & \multirow{2}{*}{80M-780M} & Classif, Gen., \\
        & & & & & & & Caption \\
        \midrule
        MolT5~\cite{molt5} & 2022.12  & LM-Centric & T5.1.1~\cite{T5} & Linearized & Transformer & 80M-780M & Gen., Cap. \\
        \midrule
        \multirow{2}{*}{KV-PLM~\cite{kvplm}} & \multirow{2}{*}{2022.01}  & \multirow{2}{*}{LM-Centric} & \multirow{2}{*}{BERT~\cite{devlin2018bert}} & \multirow{2}{*}{Linearized} & \multirow{2}{*}{N.A} & \multirow{2}{*}{110M-340M} & Classif., NER, \\
        & & & & & & & RE, Retrieval \\
        \midrule
        Chemformer~\cite{chemformer} & 2022.02  & LM-Centric & BART~\cite{bart} & Linearized & BART~\cite{bart} & 45M-230M & Regression, Gen. \\
        \midrule
        MFBERT~\cite{mfbert} & 2022.06  & LM-Centric & RoBERTa~\cite{roberta} & Linearized & N.A & 110M-340M & Classification \\
        \midrule
        MolGPT~\cite{molgpt} & 2021.10  & LM-Centric & N.A. & Linearized & GPT & 6M & Generation \\
        \midrule
        Galatica~\cite{galatica} & 2021.11  & LM-Centric & N.A. & Linearized & Transformer~\cite{vaswani2017attention} & 125M-120B & Classification \\
        \midrule
        SMILES-BERT~\cite{smilesbert} & 2019.09  & LM-Centric & Transformer~\cite{vaswani2017attention} & Linearized & N.A. & 30M-565M & Classification \\
        \midrule
        \multirow{2}{*}{MolCA~\cite{molca}} & \multirow{2}{*}{2023.10} & \multirow{2}{*}{LM-GM Aligned} & \multirow{2}{*}{Galactica} & \multirow{2}{*}{GIN} & \multirow{2}{*}{N.A} & \multirow{2}{*}{100M-877M} & Classif., Regr.,\\
        & & & & & & & Retrieval \\
        \midrule
        \multirow{2}{*}{GIT-Mol~\cite{gitmol}} & \multirow{2}{*}{2023.08} & \multirow{2}{*}{LM-GM Aligned} & \multirow{2}{*}{SciBERT~\cite{scibert}} & GIN & \multirow{2}{*}{MolT5~\cite{molt5}} & \multirow{2}{*}{190M-890M} & Classif, Gen.\\
        & & & & Linearized & & & Caption \\
        \midrule
        Prot2Text~\cite{prot2text} & 2023.07 & LM-GM Aligned & N.A. & GNN & GPT-2 & 256M-760M & Caption \\
        \midrule
        \multirow{2}{*}{MolFM~\cite{molfm}} & \multirow{2}{*}{2023.06} & \multirow{2}{*}{LM-GM Aligned} & \multirow{2}{*}{BERT~\cite{devlin2018bert}} & \multirow{2}{*}{GIN} & \multirow{2}{*}{MolT5~\cite{molt5}} & \multirow{2}{*}{61.8M} & Classif., Gen. \\
         & & & & & & & Caption, Retr. \\
        \midrule
        GIMLET~\cite{gimlet} & 2023.05 & LM-GM Aligned & T5~\cite{T5} & GT & T5~\cite{T5} & 80M-780M & Classif., Regr. \\
        \midrule
        \multirow{2}{*}{CLAMP~\cite{clamp}} & \multirow{2}{*}{2023.05} & \multirow{2}{*}{LM-GM Aligned} & BioBERT~\cite{biobert} & GNN & \multirow{2}{*}{N.A.} & \multirow{2}{*}{$\leq$11B} & Classification \\
        & & & CLIP~\cite{radford2021learning}, T5~\cite{T5} & Lin., Vec. & & & Retrieval \\
        \midrule
        MoMu-v2~\cite{momuv2} & 2023.07  & LM-GM Aligned & SciBERT~\cite{scibert} & GIN & N.A & 82M-782M & Classification \\
        \midrule
        \multirow{2}{*}{MoleculeSTM~\cite{moleculestm}} & \multirow{2}{*}{2022.12}  & \multirow{2}{*}{LM-GM Aligned} & \multirow{2}{*}{BART~\cite{bart}} & GIN & \multirow{2}{*}{BART} & \multirow{2}{*}{45M-230M} & Classif, Gen., \\
        & & & & Linearized & & & Caption \\
        \midrule
        \multirow{2}{*}{MoMu~\cite{momu}} & \multirow{2}{*}{2022.12}  & \multirow{2}{*}{LM-GM Aligned} & \multirow{1}{*}{SciBERT~\cite{scibert}} & \multirow{2}{*}{GNN} & \multirow{1}{*}{MolT5~\cite{molt5}} & \multirow{2}{*}{82M-782M} & Classif, Gen., \\
        & & & KV-PLM~\cite{kvplm} & & MoFlow~\cite{moflow} & & Caption, Retr. \\
        \midrule
        Text2Mol~\cite{text2mol} & 2021.11  & LM-GM Aligned & SciBERT~\cite{scibert} & GCN & Transformer~\cite{vaswani2017attention}  & $\geq$110M & Retrieval \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}


==> tables/6.graph-text-model.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Model collection in Section~\ref{sec:graph-text} for addressing textual information on graph levels. ``Ser.'' and ``Vec.'' represent serialized graph encoding and vectorized graph encoding. ``GC'', ``GR'', ``NER'', ``RE'', ``Ret.'', ``Gen.'', ``Cap.'' represent graph classification, graph regression, named entity recognition, relation extraction, (molecule) graph retrieval, (molecule) graph generation, (molecule) graph captioning.}
    \label{tab:graph-text-model}
    \begin{adjustbox}{width=0.99\textwidth}
    \begin{tabular}{lllllllll}
    \toprule
        Model & Time & Category & LM Encoder & LM Decoder & LM Size & Graph Encoder & Graph Decoder & Task\\
        \midrule
        MolCA~\cite{molca} & 2023.10 & Joint & Galactica & N.A & 100M-877M & GIN & N.A. & GC, Cap., Ret. \\
        \midrule
        ReLM~\cite{relm} & 2023.10 & Joint & N.A. & GPT-3.5 & N.A. & GNN & N.A. & GC (Reaction) \\ \midrule
        CatBERTa~\cite{catberta} & 2023.10 & LM-only & N.A. & RoBERTa & N.A. & Serialized & N.A. & GR \\
        \midrule
        GIT-Mol~\cite{gitmol} & 2023.08 & Joint & SciBERT & MolT5~\cite{molt5} & TODO & GIN, Ser. & N.A. & GC, Gen., Cap. \\
        \midrule
        Prot2Text~\cite{prot2text} & 2023.07 & Joint & N.A. & GPT-2 & 256M-760M & GNN & N.A. & Cap. \\
        \midrule
        LLaMA-Mol~\cite{llamamol} & 2023.07 & LLM-only & N.A. & LLaMA & 7B & Serialized & N.A. & GR, Gen. \\
        \midrule
        LLM4Mol~\cite{llm4mol} & 2023.07 & LM-only & RoBERTa & GPT-3.5 & TODO & Serialized & N.A. & GC, GR \\
        \midrule
        RT~\cite{regt} & 2023.06 & LM-only & N.A. & XLNet & N.A. & Serialized & N.A. &  GR \\
        \midrule
        MolReGPT~\cite{molregpt} & 2023.06 & LLM-only & N.A. & GPT-3.5 & N.A. & Serialized & N.A. &  Gen., Cap. \\
        \midrule
        ChatMol~\cite{chatmol} & 2023.06 & LM-only & T5 & T5 & 80M-780M & Serialized & N.A. &  Gen., Cap. \\
        \midrule
        \multirow{2}{*}{MolFM~\cite{molfm}} & \multirow{2}{*}{2023.06} & \multirow{2}{*}{Joint} & \multirow{2}{*}{BERT} & \multirow{2}{*}{MolT5~\cite{molt5}} & \multirow{2}{*}{61.8M} & \multirow{2}{*}{GIN} & \multirow{2}{*}{N.A.} & GC., Gen. \\
         & & & & & & & & Cap., Ret. \\
        \midrule
        GIMLET~\cite{gimlet} & 2023.05 & Joint & T5 & T5 & TODO & Graph Transformer & N.A. & GC, GR \\
        \midrule
        \multirow{2}{*}{CLAMP~\cite{clamp}} & \multirow{2}{*}{2023.05} & \multirow{2}{*}{Joint} & BioBERT & \multirow{2}{*}{N.A.} & \multirow{2}{*}{$\sim$11B} & GNN, & \multirow{2}{*}{N.A.} & GC, \\
        & & & CLIP, T5 & & & Ser., Vec. & & Ret. \\
        \midrule
        MolXPT~\cite{molxpt} & 2023.05 & LM-only & N.A. & GPT-2$_\text{medium}$ & 350M & Serialized & N.A. & GC, Gen. Cap. \\
        \midrule
        \multirow{3}{*}{LLM-ICL~\cite{llmicl}} & \multirow{3}{*}{2023.05} & \multirow{3}{*}{LLM-only} & \multirow{3}{*}{N.A.} & GPT-4/3.5/3 & \multirow{3}{*}{$\geq$ 780M} & \multirow{3}{*}{Serialized} & \multirow{3}{*}{N.A.} & GC, \\
        & & & & LLaMA2 & & & & Gen. \\
        & & & & Galactica & & & & Cap. \\
        \midrule
        Text+Chem T5~\cite{tct} & 2023.05 & LM-only & T5 & T5 & 80M-780M & Serialized, & N.A. & GC (Reac.), Gen., Cap. \\
        \midrule
        MoMu-v2~\cite{momuv2} & 2023.07  & Joint & SciBERT~\cite{scibert} & N.A & 82M-782M & GIN & N.A. & GC \\
        \midrule
        MoleculeSTM~\cite{moleculestm} & 2022.12  & Joint & BERT & Transformer & TOOD & GNN, Ser. & N.A. & GC, Gen., Cap. \\
        \midrule
        \multirow{2}{*}{MoMu~\cite{momu}} & \multirow{2}{*}{2022.12}  & \multirow{2}{*}{Joint} & SciBERT~\cite{scibert} & \multirow{2}{*}{MolT5~\cite{molt5}} & \multirow{2}{*}{82M-782M} & \multirow{2}{*}{GNN} & \multirow{2}{*}{MoFlow~\cite{moflow}} & {GC, Gen.,} \\
        & & & KV-PLM~\cite{kvplm} & & & & & Cap., Ret. \\
        \midrule
        MolT5~\cite{molt5} & 2022.12  & LM-only & T5.1.1~\cite{T5} & Transformer & 80M-780M & Serialized & N.A. & Gen., Cap. \\
        \midrule
        KV-PLM~\cite{kvplm} & 2022.01  & LM-only & BERT & N.A & 110M-340M & Serialized & N.A. & GC, NER, RE, Ret. \\
        \midrule
        Chemformer~\cite{chemformer} & 2022.02  & LM-only & BART~\cite{bart} & BART~\cite{bart} & 406M & Serialized & N.A. & GR, Gen. \\
        \midrule
        MFBERT~\cite{mfbert} & 2022.06  & LM-only & RoBERTa & N.A & 110M-340M & Serialized & N.A. & GC \\
        \midrule
        Text2Mol~\cite{text2mol} & 2021.11  & Joint & SciBERT~\cite{scibert} & Transformer & TODO & GCN & N.A. & Ret. \\
        \midrule
        MolGPT~\cite{molgpt} & 2021.10  & LM-only & N.A. & GPT & TODO & N.A. & N.A. & Generation \\
        \midrule
        Galatica~\cite{galatica} & 2021.11  & LLM-only & N.A. & Transformer & 125M-120B & Serialized & N.A. & GC \\
        \midrule
        SMILES-BERT~\cite{smilesbert} & 2019.09  & LM-only & N.A. & Transformer & N.A. & Serialized & N.A. & GC \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}
